Detection and Characterization of Extrasolar Planets through Mean-Motion Resonances: Simulations of Hypothetical Debris Disks

The gravitational influence of a planet on a nearby disk provides a powerful tool for detecting and studying extrasolar planetary systems. Here we demonstrate that gaps can be opened in dynamically cold debris disks at the mean-motion resonances of an orbiting planet. The gaps are opened away from the orbit of the planet itself, revealing that not all disk gaps need contain a planetary body. These gaps are large and deep enough to be detectable in resolved disk images for a wide range of reasonable disk-planet parameters, though we are not aware of any such gaps detected to date. The gap shape and size are diagnostic of the planet location, eccentricity and mass, and allow one to infer the existence of unseen planets, as well as many important parameters of both seen and unseen planets in these systems. We present expressions to allow the planetary mass to be calculated from observed gap width and location.

==> aaa.tex <==
@ARTICLE{Tamayo15,
   author = {{Tamayo}, D. and {Triaud}, A.~H.~M.~J. and {Menou}, K. and {Rein}, H.
	},
    title = "{Dynamical Stability of Imaged Planetary Systems in Formation: Application to HL Tau}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1502.05099},
 primaryClass = "astro-ph.EP",
 keywords = {celestial mechanics, planet-disk interactions, planetary systems, planets and satellites: dynamical evolution and stability, planets and satellites: formation, submillimeter: planetary systems},
     year = 2015,
    month = jun,
   volume = 805,
      eid = {100},
    pages = {100},
      doi = {10.1088/0004-637X/805/2/100},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...805..100T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nesvold15,
   author = {{Nesvold}, E.~R. and {Kuchner}, M.~J.},
    title = "{Gap Clearing by Planets in a Collisional Debris Disk}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1410.7784},
 primaryClass = "astro-ph.EP",
 keywords = {celestial mechanics, circumstellar matter, methods: numerical, planet-disk interactions, planetary systems},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {83},
    pages = {83},
      doi = {10.1088/0004-637X/798/2/83},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798...83N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cataldi15,
   author = {{Cataldi}, G. and {Brandeker}, A. and {Olofsson}, G. and {Chen}, C.~H. and 
	{Dent}, W.~R.~F. and {Kamp}, I. and {Roberge}, A. and {Vandenbussche}, B.
	},
    title = "{Constraints on the gas content of the Fomalhaut debris belt. Can gas-dust interactions explain the belt's morphology?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1412.5785},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, planetary systems, stars: individual: Fomalhaut, methods: observational, hydrodynamics, infrared: general},
     year = 2015,
    month = feb,
   volume = 574,
      eid = {L1},
    pages = {L1},
      doi = {10.1051/0004-6361/201425322},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...574L...1C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Juhasz14,
   author = {{Juhasz}, A. and {Benisty}, M. and {Pohl}, A. and {Dullemond}, C. and 
	{Dominik}, C. and {Paardekooper}, S.-J.},
    title = "{Spiral arms in scattered light images of protoplanetary discs: Are they the signposts of planets?}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1412.3412},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2014,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1412.3412J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Isella13,
   author = {{Isella}, A. and {P{\'e}rez}, L.~M. and {Carpenter}, J.~M. and 
	{Ricci}, L. and {Andrews}, S. and {Rosenfeld}, K.},
    title = "{An Azimuthal Asymmetry in the LkH{$\alpha$} 330 Disk}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1307.5848},
 primaryClass = "astro-ph.SR",
 keywords = {planet-disk interactions, protoplanetary disks, submillimeter: planetary systems, techniques: interferometric },
     year = 2013,
    month = sep,
   volume = 775,
      eid = {30},
    pages = {30},
      doi = {10.1088/0004-637X/775/1/30},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...775...30I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Kraus13,
   author = {{Kraus}, S. and {Ireland}, M. and {Sitko}, M. and {Monnier}, J. and 
	{Calvet}, N. and {Espaillat}, C. and {Grady}, C. and {Harries}, T. and 
	{Hoenig}, S. and {Russell}, R. and {Kim}, D. and {Swearing}, J. and 
	{Werren}, C. and {Wilner}, D.},
    title = "{Resolving the gap and AU-scale asymmetries in pre-transitional disks with multi-wavelength interferometry}",
booktitle = {Protostars and Planets VI Posters},
     year = 2013,
    month = jul,
    pages = {51},
   adsurl = {http://adsabs.harvard.edu/abs/2013prpl.conf2B051K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jang-Condell13,
   author = {{Jang-Condell}, H. and {Turner}, N.~J.},
    title = "{Gaps in Protoplanetary Disks as Signatures of Planets. II. Inclined Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1305.6313},
 primaryClass = "astro-ph.EP",
 keywords = {planet-disk interactions, planets and satellites: detection, protoplanetary disks, radiative transfer, stars: individual: LkCa 15 },
     year = 2013,
    month = jul,
   volume = 772,
      eid = {34},
    pages = {34},
      doi = {10.1088/0004-637X/772/1/34},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...772...34J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Debes13,
   author = {{Debes}, J.~H. and {Jang-Condell}, H. and {Weinberger}, A.~J. and 
	{Roberge}, A. and {Schneider}, G.},
    title = "{The 0.5-2.22 {$\mu$}m Scattered Light Spectrum of the Disk around TW Hya: Detection of a Partially Filled Disk Gap at 80 AU}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1306.2969},
 primaryClass = "astro-ph.EP",
 keywords = {planet-disk interactions, protoplanetary disks, radiative transfer, stars: individual: TW Hya},
     year = 2013,
    month = jul,
   volume = 771,
      eid = {45},
    pages = {45},
      doi = {10.1088/0004-637X/771/1/45},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...771...45D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanderMarel13,
   author = {{van der Marel}, N. and {van Dishoeck}, E.~F. and {Bruderer}, S. and 
	{Birnstiel}, T. and {Pinilla}, P. and {Dullemond}, C.~P. and 
	{van Kempen}, T.~A. and {Schmalzl}, M. and {Brown}, J.~M. and 
	{Herczeg}, G.~J. and {Mathews}, G.~S. and {Geers}, V.},
    title = "{A Major Asymmetric Dust Trap in a Transition Disk}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1306.1768},
 primaryClass = "astro-ph.EP",
     year = 2013,
    month = jun,
   volume = 340,
    pages = {1199-1202},
      doi = {10.1126/science.1236770},
   adsurl = {http://adsabs.harvard.edu/abs/2013Sci...340.1199V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Grady13,
   author = {{Grady}, C.~A. and {Muto}, T. and {Hashimoto}, J. and {Fukagawa}, M. and 
	{Currie}, T. and {Biller}, B. and {Thalmann}, C. and {Sitko}, M.~L. and 
	{Russell}, R. and {Wisniewski}, J. and {Dong}, R. and {Kwon}, J. and 
	{Sai}, S. and {Hornbeck}, J. and {Schneider}, G. and {Hines}, D. and 
	{Moro Mart{\'{\i}}n}, A. and {Feldt}, M. and {Henning}, T. and 
	{Pott}, J.-U. and {Bonnefoy}, M. and {Bouwman}, J. and {Lacour}, S. and 
	{Mueller}, A. and {Juh{\'a}sz}, A. and {Crida}, A. and {Chauvin}, G. and 
	{Andrews}, S. and {Wilner}, D. and {Kraus}, A. and {Dahm}, S. and 
	{Robitaille}, T. and {Jang-Condell}, H. and {Abe}, L. and {Akiyama}, E. and 
	{Brandner}, W. and {Brandt}, T. and {Carson}, J. and {Egner}, S. and 
	{Follette}, K.~B. and {Goto}, M. and {Guyon}, O. and {Hayano}, Y. and 
	{Hayashi}, M. and {Hayashi}, S. and {Hodapp}, K. and {Ishii}, M. and 
	{Iye}, M. and {Janson}, M. and {Kandori}, R. and {Knapp}, G. and 
	{Kudo}, T. and {Kusakabe}, N. and {Kuzuhara}, M. and {Mayama}, S. and 
	{McElwain}, M. and {Matsuo}, T. and {Miyama}, S. and {Morino}, J.-I. and 
	{Nishimura}, T. and {Pyo}, T.-S. and {Serabyn}, G. and {Suto}, H. and 
	{Suzuki}, R. and {Takami}, M. and {Takato}, N. and {Terada}, H. and 
	{Tomono}, D. and {Turner}, E. and {Watanabe}, M. and {Yamada}, T. and 
	{Takami}, H. and {Usuda}, T. and {Tamura}, M.},
    title = "{Spiral Arms in the Asymmetrically Illuminated Disk of MWC 758 and Constraints on Giant Planets}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1212.1466},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, instrumentation: high angular resolution, polarization, protoplanetary disks, stars: individual: MWC 758, waves},
     year = 2013,
    month = jan,
   volume = 762,
      eid = {48},
    pages = {48},
      doi = {10.1088/0004-637X/762/1/48},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...762...48G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kley12,
   author = {{Kley}, W. and {Nelson}, R.~P.},
    title = "{Planet-Disk Interaction and Orbital Evolution}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1203.1184},
 primaryClass = "astro-ph.EP",
     year = 2012,
    month = sep,
   volume = 50,
    pages = {211-249},
      doi = {10.1146/annurev-astro-081811-125523},
   adsurl = {http://adsabs.harvard.edu/abs/2012ARA%26A..50..211K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Muto12,
   author = {{Muto}, T. and {Grady}, C.~A. and {Hashimoto}, J. and {Fukagawa}, M. and 
	{Hornbeck}, J.~B. and {Sitko}, M. and {Russell}, R. and {Werren}, C. and 
	{Cur{\'e}}, M. and {Currie}, T. and {Ohashi}, N. and {Okamoto}, Y. and 
	{Momose}, M. and {Honda}, M. and {Inutsuka}, S. and {Takeuchi}, T. and 
	{Dong}, R. and {Abe}, L. and {Brandner}, W. and {Brandt}, T. and 
	{Carson}, J. and {Egner}, S. and {Feldt}, M. and {Fukue}, T. and 
	{Goto}, M. and {Guyon}, O. and {Hayano}, Y. and {Hayashi}, M. and 
	{Hayashi}, S. and {Henning}, T. and {Hodapp}, K.~W. and {Ishii}, M. and 
	{Iye}, M. and {Janson}, M. and {Kandori}, R. and {Knapp}, G.~R. and 
	{Kudo}, T. and {Kusakabe}, N. and {Kuzuhara}, M. and {Matsuo}, T. and 
	{Mayama}, S. and {McElwain}, M.~W. and {Miyama}, S. and {Morino}, J.-I. and 
	{Moro-Martin}, A. and {Nishimura}, T. and {Pyo}, T.-S. and {Serabyn}, E. and 
	{Suto}, H. and {Suzuki}, R. and {Takami}, M. and {Takato}, N. and 
	{Terada}, H. and {Thalmann}, C. and {Tomono}, D. and {Turner}, E.~L. and 
	{Watanabe}, M. and {Wisniewski}, J.~P. and {Yamada}, T. and 
	{Takami}, H. and {Usuda}, T. and {Tamura}, M.},
    title = "{Discovery of Small-scale Spiral Structures in the Disk of SAO 206462 (HD 135344B): Implications for the Physical State of the Disk from Spiral Density Wave Theory}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1202.6139},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, instrumentation: high angular resolution, polarization, protoplanetary disks, stars: individual: SAO 206462 HD 135344B, waves},
     year = 2012,
    month = apr,
   volume = 748,
      eid = {L22},
    pages = {L22},
      doi = {10.1088/2041-8205/748/2/L22},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748L..22M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kwon11,
   author = {{Kwon}, W. and {Looney}, L.~W. and {Mundy}, L.~G.},
    title = "{Resolving the Circumstellar Disk of HL Tauri at Millimeter Wavelengths}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1107.5275},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, protoplanetary disks, radio continuum: stars, stars: individual: HL Tauri, stars: pre-main sequence, techniques: interferometric},
     year = 2011,
    month = nov,
   volume = 741,
      eid = {3},
    pages = {3},
      doi = {10.1088/0004-637X/741/1/3},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741....3K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lagrange10,
   author = {{Lagrange}, A.-M. and {Bonnefoy}, M. and {Chauvin}, G. and {Apai}, D. and 
	{Ehrenreich}, D. and {Boccaletti}, A. and {Gratadour}, D. and 
	{Rouan}, D. and {Mouillet}, D. and {Lacour}, S. and {Kasper}, M.
	},
    title = "{A Giant Planet Imaged in the Disk of the Young Star {$\beta$} Pictoris}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1006.3314},
 primaryClass = "astro-ph.EP",
     year = 2010,
    month = jul,
   volume = 329,
    pages = {57-},
      doi = {10.1126/science.1187187},
   adsurl = {http://adsabs.harvard.edu/abs/2010Sci...329...57L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brown09,
   author = {{Brown}, J.~M. and {Blake}, G.~A. and {Qi}, C. and {Dullemond}, C.~P. and 
	{Wilner}, D.~J. and {Williams}, J.~P.},
    title = "{Evidence for Dust Clearing Through Resolved Submillimeter Imaging}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0909.5595},
 primaryClass = "astro-ph.SR",
 keywords = {planetary systems: protoplanetary disks, stars: pre-main sequence},
     year = 2009,
    month = oct,
   volume = 704,
    pages = {496-502},
      doi = {10.1088/0004-637X/704/1/496},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...704..496B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krivov07,
   author = {{Krivov}, A.~V. and {Queck}, M. and {L{\"o}hne}, T. and {Srem{\v c}evi{\'c}}, M.
	},
    title = "{On the nature of clumps in debris disks}",
  journal = {\aap},
   eprint = {astro-ph/0610871},
 keywords = {planetary systems: formation, circumstellar matter, meteors, meteoroids, celestial mechanics, stars: individual: {$\epsilon$} Eri.},
     year = 2007,
    month = jan,
   volume = 462,
    pages = {199-210},
      doi = {10.1051/0004-6361:20065584},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...462..199K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wyatt06,
   author = {{Wyatt}, M.~C.},
    title = "{Dust in Resonant Extrasolar Kuiper Belts: Grain Size and Wavelength Dependence of Disk Structure}",
  journal = {\apj},
   eprint = {astro-ph/0511219},
 keywords = {Celestial Mechanics, Stars: Circumstellar Matter, Stars: Planetary Systems: Formation, Stars: Individual: Name: Vega},
     year = 2006,
    month = mar,
   volume = 639,
    pages = {1153-1165},
      doi = {10.1086/499487},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...639.1153W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wyatt05,
   author = {{Wyatt}, M.~C.},
    title = "{The insignificance of P-R drag in detectable extrasolar planetesimal belts}",
  journal = {\aap},
   eprint = {astro-ph/0501038},
 keywords = {stars: circumstellar matter, stars: planetary systems: formation},
     year = 2005,
    month = apr,
   volume = 433,
    pages = {1007-1012},
      doi = {10.1051/0004-6361:20042073},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...433.1007W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wyatt03,
   author = {{Wyatt}, M.~C.},
    title = "{Resonant Trapping of Planetesimals by Planet Migration: Debris Disk Clumps and Vega's Similarity to the Solar System}",
  journal = {\apj},
   eprint = {astro-ph/0308253},
 keywords = {Celestial Mechanics, Stars: Circumstellar Matter, Stars: Planetary Systems: Formation, Stars: Planetary Systems: Protoplanetary Disks, Stars: Individual: Name: Vega},
     year = 2003,
    month = dec,
   volume = 598,
    pages = {1321-1340},
      doi = {10.1086/379064},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...598.1321W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilner02,
   author = {{Wilner}, D.~J. and {Holman}, M.~J. and {Kuchner}, M.~J. and 
	{Ho}, P.~T.~P.},
    title = "{Structure in the Dusty Debris around Vega}",
  journal = {\apjl},
   eprint = {astro-ph/0203264},
 keywords = {Celestial Mechanics, Stars: Circumstellar Matter, Stars: Planetary Systems: Protoplanetary Disks, Stars: Individual: Constellation Name: {$\alpha$} Lyrae},
     year = 2002,
    month = apr,
   volume = 569,
    pages = {L115-L119},
      doi = {10.1086/340691},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...569L.115W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Augereau01,
   author = {{Augereau}, J.~C. and {Nelson}, R.~P. and {Lagrange}, A.~M. and 
	{Papaloizou}, J.~C.~B. and {Mouillet}, D.},
    title = "{Dynamical modeling of large scale asymmetries in the beta Pictoris dust disk}",
  journal = {\aap},
   eprint = {astro-ph/0102069},
 keywords = {STARS: CIRCUMSTELLAR MATTER, STARS: BETA PICTORIS},
     year = 2001,
    month = may,
   volume = 370,
    pages = {447-455},
      doi = {10.1051/0004-6361:20010199},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...370..447A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Heap00,
   author = {{Heap}, S.~R. and {Lindler}, D.~J. and {Lanz}, T.~M. and {Cornett}, R.~H. and 
	{Hubeny}, I. and {Maran}, S.~P. and {Woodgate}, B.},
    title = "{Space Telescope Imaging Spectrograph Coronagraphic Observations of {$\beta$} Pictoris}",
  journal = {\apj},
 keywords = {Accretion, Accretion Disks, Stars: Circumstellar Matter, Stars: Planetary Systems, Stars: Imaging, stars: individual ({$\beta$} Pictoris)},
     year = 2000,
    month = aug,
   volume = 539,
    pages = {435-444},
      doi = {10.1086/309188},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...539..435H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Murray99,
   author = {{Murray}, C.~D. and {Dermott}, S.~F.},
    title = "{Solar system dynamics}",
booktitle = {Solar system dynamics by Murray, C.~D., 1999},
     year = 1999,
   adsurl = {http://adsabs.harvard.edu/abs/1999ssd..book.....M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Fridman99,
   author = {{Fridman}, Gorkavyl, Nikolai N., A.~M.},
    title = "{Physics of Planetary Rings. Celestial Mechanics of Continuous Media.}",
booktitle = {Physics of Planetary Rings.~Celestial Mechanics of Continuous Media.~Fridman, Alexei M., Gorkavyi, Nikolai N., pp.~436.~ISBN 3-540-64864-X.~Springer-Verlag Berlin Heidelberg 1999},
     year = 1999,
   adsurl = {http://adsabs.harvard.edu/abs/1999ppr..book.....F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mouillet97,
   author = {{Mouillet}, D. and {Larwood}, J.~D. and {Papaloizou}, J.~C.~B. and 
	{Lagrange}, A.~M.},
    title = "{A planet on an inclined orbit as an explanation of the warp in the Beta Pictoris disc}",
  journal = {\mnras},
   eprint = {astro-ph/9705100},
 keywords = {Planetary Orbits, Stellar Orbits, Stellar Envelopes, Extrasolar Planets, Warpage, Adaptive Optics, Companion Stars},
     year = 1997,
    month = dec,
   volume = 292,
    pages = {896},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.292..896M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Burrows95,
   author = {{Burrows}, C.~J. and {Krist}, J.~E. and {Stapelfeldt}, K.~R. and 
	{WFPC2 Investigation Definition Team}},
    title = "{HST Observations of the Beta Pictoris Circumstellar Disk}",
booktitle = {American Astronomical Society Meeting Abstracts},
     year = 1995,
   series = {Bulletin of the American Astronomical Society},
   volume = 27,
    month = dec,
    pages = {1329},
   adsurl = {http://adsabs.harvard.edu/abs/1995AAS...187.3205B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kalas95,
   author = {{Kalas}, P. and {Jewitt}, D.},
    title = "{Asymmetries in the Beta Pictoris Dust Disk}",
  journal = {\aj},
 keywords = {STARS: INDIVIDUAL: BETA PICTORIS, CIRCUMSTELLAR MATTER},
     year = 1995,
    month = aug,
   volume = 110,
    pages = {794},
      doi = {10.1086/117565},
   adsurl = {http://adsabs.harvard.edu/abs/1995AJ....110..794K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ida93,
   author = {{Ida}, S. and {Makino}, J.},
    title = "{Scattering of planetesimals by a protoplanet - Slowing down of runaway growth}",
  journal = {Icarus},
 keywords = {Protoplanets, Mass Distribution, Planetary Evolution, Many Body Problem, Computerized Simulation, Scattering, Spatial Distribution, Mass Ratios},
     year = 1993,
    month = nov,
   volume = 106,
    pages = {210},
      doi = {10.1006/icar.1993.1167},
   adsurl = {http://adsabs.harvard.edu/abs/1993Icar..106..210I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wisdom91,
   author = {{Wisdom}, J. and {Holman}, M.},
    title = "{Symplectic maps for the n-body problem}",
  journal = {\aj},
 keywords = {Many Body Problem, Planetary Evolution, Pluto (Planet), Astronomical Maps, Gravitational Effects},
     year = 1991,
    month = oct,
   volume = 102,
    pages = {1528-1538},
      doi = {10.1086/115978},
   adsurl = {http://adsabs.harvard.edu/abs/1991AJ....102.1528W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Smith84,
   author = {{Smith}, B.~A. and {Terrile}, R.~J.},
    title = "{A circumstellar disk around Beta Pictoris}",
  journal = {Science},
 keywords = {Dwarf Stars, Main Sequence Stars, Planetary Evolution, Stellar Envelopes, Brightness, Disks, Infrared Astronomy Satellite, Scattering Cross Sections, Visible Spectrum},
     year = 1984,
    month = dec,
   volume = 226,
    pages = {1421-1424},
      doi = {10.1126/science.226.4681.1421},
   adsurl = {http://adsabs.harvard.edu/abs/1984Sci...226.1421S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Aumann84,
   author = {{Aumann}, H.~H. and {Beichman}, C.~A. and {Gillett}, F.~C. and 
	{de Jong}, T. and {Houck}, J.~R. and {Low}, F.~J. and {Neugebauer}, G. and 
	{Walker}, R.~G. and {Wesselius}, P.~R.},
    title = "{Discovery of a shell around Alpha Lyrae}",
  journal = {\apjl},
 keywords = {A Stars, Infrared Astronomy, Reference Stars, Stellar Envelopes, Emission Spectra, Infrared Astronomy Satellite, Particle Production, Spaceborne Astronomy, Thermal Radiation},
     year = 1984,
    month = mar,
   volume = 278,
    pages = {L23-L27},
      doi = {10.1086/184214},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...278L..23A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Shu84,
   author = {{Shu}, F.~H.},
    title = "{Waves in planetary rings}",
 keywords = {Celestial Mechanics, Density Wave Model, Gravity Waves, Planetary Rings, Saturn Rings, Natural Satellites, Orbital Mechanics, Particle Density (Concentration), Resonance, Spiral Galaxies, Viscosity, Wave Excitation},
booktitle = {IAU Colloq. 75: Planetary Rings},
     year = 1984,
   editor = {{Greenberg}, R. and {Brahic}, A.},
    pages = {513-561},
   adsurl = {http://adsabs.harvard.edu/abs/1984prin.conf..513S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Holberg82,
   author = {{Holberg}, J.~B. and {Forrester}, W.~T. and {Lissauer}, J.~J.
	},
    title = "{Identification of resonance features within the rings of Saturn}",
  journal = {\nat},
 keywords = {Resonance, Saturn Rings, Saturn Satellites, Stellar Occultation, Ultraviolet Astronomy, Optical Thickness, Planetary Orbits, Voyager 2 Spacecraft, Wave Propagation, SATURN, RINGS, RESONANCE, FEATURES, VOYAGER 2, ULTRAVIOLET, WAVELENGTHS, SPECTROMETER, OCCULTATIONS, OPTICAL PROPERTIES, DEPTH, DENSITY WAVES, PATTERNS, ANALYSIS, DENSITY, SURFACE, MASS, C RING, DISTANCE, SOURCE, SATELLITES, 1980S27, 1980S26, 1980S1, MIMAS, TITAN, HYPERION, IAPETUS, BOUNDARIES, ORIGIN, MORPHOLOGY, CASSINI DIVISION, A RING, B RING, DATA},
     year = 1982,
    month = may,
   volume = 297,
    pages = {115-120},
      doi = {10.1038/297115a0},
   adsurl = {http://adsabs.harvard.edu/abs/1982Natur.297..115H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lane82,
   author = {{Lane}, A.~L. and {Hord}, C.~W. and {West}, R.~A. and {Esposito}, L.~W. and 
	{Coffeen}, D.~L. and {Sato}, M. and {Simmons}, K.~E. and {Pomphrey}, R.~B. and 
	{Morris}, R.~B.},
    title = "{Photopolarimetry from Voyager 2 - Preliminary results on Saturn, Titan, and the rings}",
  journal = {Science},
 keywords = {Polarimeters, Saturn Atmosphere, Saturn Rings, Titan, Voyager 2 Spacecraft, Encke Method, Limb Brightening, Polarization Characteristics, Saturn Satellites, Stellar Occultation, Ultraviolet Spectrophotometers, DYNAMICS, COMPARISONS, PPS, PHOTOMETRY, EQUIPMENT, PROCEDURE, B RING, DENSITY, VISCOSITY, ANALYSIS, SATURN, VOYAGER 2, PHOTOPOLARIMETER, SATELLITES, TITAN, RINGS, ATMOSPHERE, LIMBS, BRIGHTNESS, ULTRAVIOLET, WAVELENGTHS, COLORS, POLARIZATION, OPACITY, OPTICAL PROPERTIES, MODELS, PARTICLES, OCCULTATIONS, THICKNESS, DENSITY WAVES, RESONANCE, F RING, ENCKE DIVISIONS, SIZE, MAPS, DATA, PHOTOGRAPHS, IMAGERY, DEPTH},
     year = 1982,
    month = jan,
   volume = 215,
    pages = {537-543},
      doi = {10.1126/science.215.4532.537},
   adsurl = {http://adsabs.harvard.edu/abs/1982Sci...215..537L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reche08,
   author = {{Reche}, R. and {Beust}, H. and {Augereau}, J.-C. and {Absil}, O.
	},
    title = "{On the observability of resonant structures in planetesimal disks due to planetary migration}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0801.2691},
 keywords = {method: N-body simulations, celestial mechanics, stars: planetary systems, stars: individual: <ASTROBJ>Vega</ASTROBJ>},
     year = 2008,
    month = mar,
   volume = 480,
    pages = {551-561},
      doi = {10.1051/0004-6361:20077934},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...480..551R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Kirkwood67,
   author = {{Kirkwood}, D.},
    title = "{Meteoric astronomy: a treatise on shooting-stars, fireballs, and aerolites.}",
 keywords = {METEORS},
booktitle = {Philadelphia, J.~B.~Lippincott {\amp} co., 1867.},
     year = 1867,
   adsurl = {http://adsabs.harvard.edu/abs/1867QB741.K59......},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chiang09,
   author = {{Chiang}, E. and {Kite}, E. and {Kalas}, P. and {Graham}, J.~R. and 
	{Clampin}, M.},
    title = "{Fomalhaut's Debris Disk and Planet: Constraining the Mass of Fomalhaut b from disk Morphology}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0811.1985},
 keywords = {celestial mechanics, circumstellar matter, planetary systems, planetary systems: protoplanetary disks, stars: individual: Fomalhaut},
     year = 2009,
    month = mar,
   volume = 693,
    pages = {734-749},
      doi = {10.1088/0004-637X/693/1/734},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...693..734C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stark09,
   author = {{Stark}, C.~C. and {Kuchner}, M.~J.},
    title = "{A New Algorithm for Self-consistent Three-dimensional Modeling of Collisions in Dusty Debris Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0909.2227},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, interplanetary medium, methods: N-body simulations, methods: numerical, planetary systems},
     year = 2009,
    month = dec,
   volume = 707,
    pages = {543-553},
      doi = {10.1088/0004-637X/707/1/543},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...707..543S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@webpage{NRAO14,
	Author = {NRAO},
	Date-Added = {2015-09-22 23:35:07 +0000},
	Date-Modified = {2015-09-24 17:36:44 +0000},
	Lastchecked = {2015},
	Month = {November},
	Read = {1},
	Title = {Birth of Planets Revealed in Astonishing Detail in ALMA's 'Best Image Ever', National Radio Astronomy Observatory (Press Release)},
	Url = {http://public.nrao.edu/news/pressreleases/planet-formation-alma},
	Urldate = {2015},
	Year = {2014},
}


@webpage{AstDyS,
	Author = {AstDyS},
	Date-Added = {2015-09-22 23:35:07 +0000},
	Date-Modified = {2015-09-24 17:36:44 +0000},
	Lastchecked = {2015},
	Month = {November},
	Read = {1},
	Title = {Asteroids Dynamic Site, (http://hamilton.dm.unipi.it/astdys/)},
	Url = {http://hamilton.dm.unipi.it/astdys/},
	Urldate = {2015},
	Year = {2015},
}


@ARTICLE{Kuchner03,
   author = {{Kuchner}, M.~J. and {Holman}, M.~J.},
    title = "{The Geometry of Resonant Signatures in Debris Disks with Planets}",
  journal = {\apj},
   eprint = {astro-ph/0209261},
 keywords = {Celestial Mechanics, Stars: Circumstellar Matter, Interplanetary Medium, Stars: Planetary Systems, Stars: Individual: Constellation Name: {$\alpha$} Lyrae, Stars: Individual: Constellation Name: {$\epsilon$} Eridani, Stars: Individual: Name: Fomalhaut},
     year = 2003,
    month = may,
   volume = 588,
    pages = {1110-1120},
      doi = {10.1086/374213},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...588.1110K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

